How Do Viewers Synthesize Conflicting Information from Data Visualizations?

Scientific knowledge develops through cumulative discoveries that build on, contradict, contextualize, or correct prior findings. Scientists and journalists often communicate these incremental findings to lay people through visualizations and text (e.g., the positive and negative effects of caffeine intake). Consequently, readers need to integrate diverse and contrasting evidence from multiple sources to form opinions or make decisions. However, the underlying mechanism for synthesizing information from multiple visualizations remains underexplored. To address this knowledge gap, we conducted a series of four experiments (N = 1166) in which participants synthesized empirical evidence from a pair of line charts presented sequentially. In Experiment 1, we administered a baseline condition with charts depicting no specific context where participants held no strong belief. To test for the generalizability, we introduced real-world scenarios to our visualizations in Experiment 2, and added accompanying text descriptions similar to on-line news articles or blog posts in Experiment 3. In all three experiments, we varied the relative direction and magnitude of line slopes within the chart pairs. We found that participants tended to weigh the positive slope more when the two charts depicted relationships in the opposite direction (e.g., one positive slope and one negative slope). Participants tended to weigh the less steep slope when the two charts depicted relationships in the same direction (e.g., both positive). Through these experiments, we characterize participants' synthesis behaviors depending on the relationship between the information they viewed, contribute to theories describing underlying cognitive mechanisms in information synthesis, and describe design implications for data storytelling.

==> 98_figures_tables.tex <==

% Date and time: Fri, Mar 18, 2022 - 05:02:22
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Effect of having a strong slope\\ Response slope taken from user input on widget} 
  \label{Effect_Negative_Slope} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from mathematical average} \\ 
\hline \\[-1.8ex] 
 High Positive Slope & 0.106 \\ 
  & (0.064) \\ 
  High Negative Slope & 0.292^{***} \\ 
  & (0.060) \\ 
  Constant & -0.135^{*} \\ 
  & (0.069) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{234} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.127} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.120} \\ 
\hline 
\hline \\[-1.8ex]
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 




% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Effect of the greater slope if presented second \\ Response slope taken from user input on widget} 
  \label{SecondGreaterSlope} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from greater slope} \\ 
\hline \\[-1.8ex] 
 Second slope is greater & -0.173^{**} \\ 
  & (0.069) \\ 
  Constant & -0.322^{***} \\ 
  & (0.049) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{234} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.027} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.023} \\ 
\hline 
\hline \\[-1.8ex]
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 





% Date and time: Sat, Mar 19, 2022 - 00:00:56
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Triangulation: Effect of having a strong slope \\ Response slope computed through user inputs from text-boxes} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from mathematical average} \\ 
\hline \\[-1.8ex] 
 High Positive Slope & 1.617^{***} \\ 
  & (0.371) \\ 
  High Negative Slope & -0.344 \\ 
  & (0.346) \\ 
  Constant & 0.076 \\ 
  & (0.405) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{252} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.182} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.176} \\ 
\hline 
\hline \\[-1.8ex]
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

%Date and time: Sat, Mar 19, 2022 - 00:04:55
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Triangulation: Effect of greater slope if presented second \\ Response slope computed through user inputs from text-boxes} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from greater slope} \\ 
\hline \\[-1.8ex] 
 Second slope is greater & -1.175^{***} \\ 
  & (0.427) \\ 
  Constant & 1.681^{***} \\ 
  & (0.311) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{219} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.034} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.029} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 
 \\
 \\




% Date and time: Sat, Mar 19, 2022 - 01:48:04
\begin{table}[!htbp] \centering 
  \caption{Student's t-test for comparison between widget input slopes and computed slopes} 
  \label{} 
  \rotatebox{90}{
\begin{tabular}{@{\extracolsep{5pt}} cccccccc} 
\hline \\[-1.8ex] 
condition\_full & estimate & estimate1 & estimate2 & statistic & p\_value & method & alternative \\ 
\hline \\[-1.8ex] 
11  -  High Positive and Medium Positive & -0.308 & 0.414 & 0.721 & c(t = -4.715) & \textasteriskcentered \textasteriskcentered \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
12  -  Medium Positive and High Positive & -0.261 & 0.422 & 0.684 & c(t = -4.172) & \textasteriskcentered \textasteriskcentered \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
21  -  High Negative and Medium Negative & 0.03 & -0.21 & -0.24 & c(t = 0.216) &  & Welch Two Sample t-test & two.sided \\ 
22  -  Medium Negative and High Negative & -0.062 & -0.335 & -0.273 & c(t = -0.439) &  & Welch Two Sample t-test & two.sided \\ 
31  -  High Negative and High Positive & -0.098 & 0.246 & 0.344 & c(t = -0.742) &  & Welch Two Sample t-test & two.sided \\ 
32  -  High Positive and High Negative & 0.048 & 0.24 & 0.192 & c(t = 0.361) &  & Welch Two Sample t-test & two.sided \\ 
41  -  High Positive and Medium Negative & -0.199 & 0.322 & 0.522 & c(t = -2.177) & \textasteriskcentered \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
42  -  Medium Negative and High Positive & -0.242 & 0.11 & 0.352 & c(t = -2.991) & \textasteriskcentered \textasteriskcentered \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
51  -  High Positive and Low Negative & -0.248 & 0.274 & 0.522 & c(t = -3.228) & \textasteriskcentered \textasteriskcentered \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
52  -  Low Negative and High Positive & -0.211 & 0.184 & 0.395 & c(t = -1.709) & \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
61  -  High Negative and Low Positive & -0.05 & 0.1 & 0.15 & c(t = -0.585) &  & Welch Two Sample t-test & two.sided \\ 
62  -  Low Positive and High Negative & 0.121 & -0.207 & -0.328 & c(t = 1.087) &  & Welch Two Sample t-test & two.sided \\ 
\hline \\[-1.8ex]
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular}  
}
\end{table} 
% Date and time: Sat, Mar 19, 2022 - 02:25:25
\begin{table}[!htbp] \centering 
  \caption{Student's t-test for comparison between the value for crop yield estimation for 20 inches of water using widget input slopes and text-boxes} 
  \label{} 
    \rotatebox{90}{
\begin{tabular}{@{\extracolsep{5pt}} cccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
condition\_full & estimate & estimate1 & estimate2 & statistic & p\_value & method & alternative \\ 
\hline \\[-1.8ex] 
11  -  High Positive and Medium Positive & 8.334 & 36.054 & 27.72 & c(t = 2.336) & \textasteriskcentered \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
12  -  Medium Positive and High Positive & 6.077 & 37.491 & 31.414 & c(t = 2.166) & \textasteriskcentered \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
21  -  High Negative and Medium Negative & -2.21 & 54.135 & 56.345 & c(t = -0.523) &  & Welch Two Sample t-test & two.sided \\ 
22  -  Medium Negative and High Negative & 1.658 & 57.467 & 55.81 & c(t = 0.325) &  & Welch Two Sample t-test & two.sided \\ 
31  -  High Negative and High Positive & 0.877 & 39.982 & 39.105 & c(t = 0.187) &  & Welch Two Sample t-test & two.sided \\ 
32  -  High Positive and High Negative & 3.254 & 42.344 & 39.091 & c(t = 0.647) &  & Welch Two Sample t-test & two.sided \\ 
41  -  High Positive and Medium Negative & 5.624 & 36.774 & 31.15 & c(t = 1.891) & \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
42  -  Medium Negative and High Positive & 4.198 & 42.531 & 38.333 & c(t = 1.394) &  & Welch Two Sample t-test & two.sided \\ 
51  -  High Positive and Low Negative & 10.147 & 41.933 & 31.786 & c(t = 4.251) & \textasteriskcentered \textasteriskcentered \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
52  -  Low Negative and High Positive & -0.69 & 38.428 & 39.118 & c(t = -0.171) &  & Welch Two Sample t-test & two.sided \\ 
61  -  High Negative and Low Positive & 1.94 & 43.887 & 41.947 & c(t = 0.508) &  & Welch Two Sample t-test & two.sided \\ 
62  -  Low Positive and High Negative & -4.181 & 55.776 & 59.957 & c(t = -1.097) &  & Welch Two Sample t-test & two.sided \\ 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular}
}
\end{table} 


\begin{table}[!htbp] \centering 
  \caption{Student's t-test for comparison between the value for crop yield estimation for 80 inches of water using widget input slopes and text-boxes} 
  \label{} 
      \rotatebox{90}{
\begin{tabular}{@{\extracolsep{5pt}} cccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
condition\_full & estimate & estimate1 & estimate2 & statistic & p\_value & method & alternative \\ 
\hline \\[-1.8ex] 
11  -  High Positive and Medium Positive & -10.13 & 60.87 & 71 & c(t = -2.89) & \textasteriskcentered \textasteriskcentered \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
12  -  Medium Positive and High Positive & -9.613 & 62.835 & 72.448 & c(t = -3.219) & \textasteriskcentered \textasteriskcentered \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
21  -  High Negative and Medium Negative & -0.396 & 41.535 & 41.931 & c(t = -0.08) &  & Welch Two Sample t-test & two.sided \\ 
22  -  Medium Negative and High Negative & -2.047 & 37.381 & 39.429 & c(t = -0.477) &  & Welch Two Sample t-test & two.sided \\ 
31  -  High Negative and High Positive & -4.976 & 54.761 & 59.737 & c(t = -0.994) &  & Welch Two Sample t-test & two.sided \\ 
32  -  High Positive and High Negative & 6.135 & 56.772 & 50.636 & c(t = 1.433) &  & Welch Two Sample t-test & two.sided \\ 
41  -  High Positive and Medium Negative & -6.326 & 56.124 & 62.45 & c(t = -1.306) &  & Welch Two Sample t-test & two.sided \\ 
42  -  Medium Negative and High Positive & -10.326 & 49.102 & 59.429 & c(t = -2.44) & \textasteriskcentered \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
51  -  High Positive and Low Negative & -4.738 & 58.369 & 63.107 & c(t = -1.472) &  & Welch Two Sample t-test & two.sided \\ 
52  -  Low Negative and High Positive & -13.349 & 49.475 & 62.824 & c(t = -2.075) & \textasteriskcentered \textasteriskcentered  & Welch Two Sample t-test & two.sided \\ 
61  -  High Negative and Low Positive & -1.06 & 49.887 & 50.947 & c(t = -0.272) &  & Welch Two Sample t-test & two.sided \\ 
62  -  Low Positive and High Negative & 3.071 & 43.332 & 40.261 & c(t = 0.647) &  & Welch Two Sample t-test & two.sided \\ 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} }
\end{table} 



% Date and time: Sat, Mar 19, 2022 - 02:34:11
\begin{table}[!htbp] \centering 
  \caption{Student's t-test for comparison between the value for crop yield estimation for 50 inches of water using widget input slopes and text-boxes} 
  \label{} 
   \rotatebox{90}{
\begin{tabular}{@{\extracolsep{5pt}} cccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
condition\_full & estimate & estimate1 & estimate2 & statistic & p\_value & method & alternative \\ 
\hline \\[-1.8ex] 
11  -  High Positive and Medium Positive & 26.795 & 73.835 & 47.04 & c(t = 1.195) &  & Welch Two Sample t-test & two.sided \\ 
12  -  Medium Positive and High Positive & -81.921 & -31.439 & 50.483 & c(t = -1.042) &  & Welch Two Sample t-test & two.sided \\ 
21  -  High Negative and Medium Negative & 47.311 & 89.828 & 42.517 & c(t = 1.194) &  & Welch Two Sample t-test & two.sided \\ 
22  -  Medium Negative and High Negative & -5.011 & 43.275 & 48.286 & c(t = -0.817) &  & Welch Two Sample t-test & two.sided \\ 
31  -  High Negative and High Positive & 41.892 & 90.524 & 48.632 & c(t = 1.737) &  & Welch Two Sample t-test & two.sided \\ 
32  -  High Positive and High Negative & -448026491427565 & -448026491427513 & 51.909 & c(t = -1) &  & Welch Two Sample t-test & two.sided \\ 
41  -  High Positive and Medium Negative & 4.89 & 55.44 & 50.55 & c(t = 0.439) &  & Welch Two Sample t-test & two.sided \\ 
42  -  Medium Negative and High Positive & 17.737 & 69.879 & 52.143 & c(t = 0.957) &  & Welch Two Sample t-test & two.sided \\ 
51  -  High Positive and Low Negative & 1.41 & 51.41 & 50 & c(t = 0.341) &  & Welch Two Sample t-test & two.sided \\ 
52  -  Low Negative and High Positive & -0.562 & 47.849 & 48.412 & c(t = -0.047) &  & Welch Two Sample t-test & two.sided \\ 
61  -  High Negative and Low Positive & 7.838 & 55.206 & 47.368 & c(t = 0.507) &  & Welch Two Sample t-test & two.sided \\ 
62  -  Low Positive and High Negative & -8.521 & 37.609 & 46.13 & c(t = -0.624) &  & Welch Two Sample t-test & two.sided \\ 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} }
\end{table}

% Date and time: Sat, Mar 19, 2022 - 06:21:39
\begin{table}[!htbp] \centering 
  \caption{Agreement on decision choice using responses from widget, text-boxes, decision task, and mathematical average } 
  \label{} 
  \rotatebox{90}{
\begin{tabular}{@{\extracolsep{5pt}} ccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Condition & Average-Widget & Average-Text & Average-Decision & Widget-Text & Widget-Decision & Text-Decision \\ 
\hline \\[-1.8ex] 
11  -  High Positive and Medium Positive & 1 & 0.8 & 0.84 & 0.8 & 0.84 & 0.72 \\ 
12  -  Medium Positive and High Positive & 1 & 0.9 & 0.86 & 0.9 & 0.86 & 0.83 \\ 
21  -  High Negative and Medium Negative & 0 & 0.03 & 0.72 & 0.97 & 0.28 & 0.24 \\ 
22  -  Medium Negative and High Negative & 0 & 0.05 & 0.67 & 0.95 & 0.33 & 0.29 \\ 
31  -  High Negative and High Positive & 1 & 1 & 0.74 & 1 & 0.74 & 0.74 \\ 
32  -  High Positive and High Negative & 1 & 0.95 & 0.77 & 0.95 & 0.77 & 0.73 \\ 
41  -  High Positive and Medium Negative & 1 & 1 & 0.65 & 1 & 0.65 & 0.65 \\ 
42  -  Medium Negative and High Positive & 1 & 1 & 0.76 & 1 & 0.76 & 0.76 \\ 
51  -  High Positive and Low Negative & 1 & 0.93 & 0.89 & 0.93 & 0.89 & 0.82 \\ 
52  -  Low Negative and High Positive & 1 & 1 & 0.71 & 1 & 0.71 & 0.71 \\ 
61  -  High Negative and Low Positive & 0 & 0 & 0.53 & 1 & 0.47 & 0.47 \\ 
62  -  Low Positive and High Negative & 0 & 0 & 0.57 & 1 & 0.43 & 0.43 \\ 
\hline \\[-1.8ex] 
\hline \\[-1.8ex] 
Order & Average-Widget & Average-Text & Average-Decision & Widget-Text & Widget-Decision & Text-Decision \\ 
\hline \\[-1.8ex] 
Larger slope first & 0.66 & 0.61 & 0.74 & 0.94 & 0.64 & 0.6 \\ 
Larger slope last & 0.67 & 0.65 & 0.73 & 0.96 & 0.65 & 0.63 \\ 
\hline \\[-1.8ex]
\hline \\[-1.8ex] 
\end{tabular}   
}
\end{table} 

% Date and time: Sun, Mar 20, 2022 - 15:10:26
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Effect of difference in stimuli slopes on the distance of the response from the mathematical average} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from mathematical average} \\ 
\hline \\[-1.8ex] 
 Difference in stimuli slopes & 0.145^{**} \\ 
  & (0.070) \\ 
  Constant & -0.039 \\ 
  & (0.055) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{232} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.018} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.014} \\ 
\hline 
\hline \\[-1.8ex]
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


% Date and time: Sun, Mar 20, 2022 - 15:24:57
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from mathematical average} \\ 
\hline \\[-1.8ex] 
 Difference in stimuli slopes & -0.173^{**} \\ 
  & (0.069) \\ 
  Prior & -0.300^{***} \\ 
  & (0.076) \\ 
  Constant & 0.144^{**} \\ 
  & (0.058) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{234} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.084} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.076} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

% Date and time: Sun, Mar 20, 2022 - 22:18:42
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from larger slope} \\ 
\hline \\[-1.8ex] 
 Larger Slope & -0.239^{***} \\ 
  & (0.048) \\ 
  Smaller Slope & 0.230^{**} \\ 
  & (0.108) \\ 
  Constant & 0.696^{***} \\ 
  & (0.033) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{273} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.108} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.101} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


% Date and time: Sun, Mar 20, 2022 - 22:24:51
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from larger slope} \\ 
\hline \\[-1.8ex] 
 Larger Slope & -0.242^{***} \\ 
  & (0.048) \\ 
  Smaller Slope & 0.244^{**} \\ 
  & (0.110) \\ 
  Age & -0.0002 \\ 
  & (0.002) \\ 
  Gender (Male) & -0.049 \\ 
  & (0.060) \\ 
  Score (Attitude towards science) & 0.007 \\ 
  & (0.008) \\ 
  Score (Visual literacy) & -0.004 \\ 
  & (0.007) \\ 
  Constant & 0.621^{***} \\ 
  & (0.218) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{273} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.113} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.093} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 



% Date and time: Sun, Mar 20, 2022 - 22:21:13
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from Negative slope} \\ 
\hline \\[-1.8ex] 
 Positive Slope & -0.192 \\ 
  & (0.125) \\ 
  Negative Slope & -0.445^{***} \\ 
  & (0.129) \\ 
  Constant & 0.521^{***} \\ 
  & (0.105) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{169} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.155} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.145} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 




% Date and time: Sun, Mar 20, 2022 - 22:18:16
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from Negative slope} \\ 
\hline \\[-1.8ex] 
 Positive Slope & -0.177 \\ 
  & (0.129) \\ 
  Negative Slope & -0.460^{***} \\ 
  & (0.132) \\ 
  Age & -0.0003 \\ 
  & (0.002) \\ 
  Gender (Male) & 0.020 \\ 
  & (0.054) \\ 
  Score (Attitude towards science) & -0.005 \\ 
  & (0.008) \\ 
  Score (Visual literacy) & 0.006 \\ 
  & (0.006) \\ 
  Constant & 0.541^{**} \\ 
  & (0.226) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{169} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.161} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.130} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


% Date and time: Mon, Mar 21, 2022 - 00:09:38
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from first stimuli} \\ 
\hline \\[-1.8ex] 
 Difference in stimuli slopes & -0.190^{*} \\ 
  & (0.107) \\ 
  Constant & 0.677^{***} \\ 
  & (0.083) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{269} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.012} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.008} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 



% Date and time: Fri, Mar 25, 2022 - 11:29:42
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Exp 3: Effects of having a strong slope \\ Response slope taken from user input on widget} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from mathematical average} \\ 
\hline \\[-1.8ex] 
 High Positive Slope & 0.080 \\ 
  & (0.049) \\ 
  High Negative Slope & 0.333^{***} \\ 
  & (0.046) \\ 
  Political Affiliation (Repub.) & -0.072^{**} \\ 
  & (0.031) \\ 
  Constant & -0.018 \\ 
  & (0.054) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{282} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.237} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.229} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 



% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Effect of greater slope if presented second \\ Response slope computed through user input on widget} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Distance from greater slope} \\ 
\hline \\[-1.8ex] 
 Second slope is greater & 0.051 \\ 
  & (0.062) \\ 
  Political Affiliation: Republican & 0.029 \\ 
  & (0.062) \\ 
  Constant & 0.575^{***} \\ 
  & (0.055) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{282} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.003} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{-0.004} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

\begin{figure*}
  \includegraphics[width=\textwidth,height=5in]{Figures/Findings1_temp.png}
  \caption{}
\end{figure*}                    

\begin{figure*}
  \includegraphics[width=\textwidth,height=5in]{Figures/normalisedDistance_fromLarger_Mar20_corrected.png}
  \caption{}
\end{figure*}  

\begin{figure*}
  \includegraphics[width=\textwidth,height=\textwidth]{Figures/normalisedDistance_computedSlope_temp.png}
  \caption{}
\end{figure*}  
% \includepdf{Figures/Findings1_temp.png}
% \includepdf{Figures/normalisedDistance_withoutDensity_temp.png}
% \includepdf{Figures/normalisedDistance_computedSlope_temp.png}
%% \includepdf{Figures/distanceFrom_greaterSlope_temp.png}



==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
last modified by Bernhard Finkbeiner, July 5, 2010

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored by
the IEEE Visualization & Graphics Technical Committee (VGTC).

The only conferences that use the 'journal' document option:
- IEEE Visualization Conference (Research and Application Papers Only)
- IEEE Information Visualization Conference (Research and Application
Papers Only)

It contains 13 files:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed,
                  somewhere in the TeX search path
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
sample.eps      - an image used by the example paper
sample.pdf      - its PDF version
template-journal*.pdf    - an example proper pdf output in default
                          conference mode, with and without teaser
CypressView.eps - teaser image
CypressView.pdf - its PDF version
makefile     - makefile including bibtex compilation and proper PDF
                generation

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We
suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create
a file called 'template.pdf'. Please make sure, that its layout is
identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process
manually.  Below are a list of available options that may be passed to
make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> scratch.tex <==
\section{Related Work}


% As a society, we are increasingly concerned about making data-driven decisions. 
% Specifically, if they already have a pre-existing stance on the question they are trying to search more information for, they might fall victim to positive confirmation bias, which is a tendency to search for evidence which could confirm that belief, rather than for evidence which could disconfirm it \cite{jones2001positive, Wason1968Rule}. 

% However, scientists are not completely unbiased when synthesizing information, 

% To tackle this idproblem, researchers have called for systematic reviewing guidelines and meta-analysis to enforce statistical procedure for synthesizing findings. 




% However, scientists are not completely unbiased when synthesizing information; for example, when writing a review, the collection and interpretation of research articles is a largely idiosyncratic process  \cite{greenhalgh1997read}.

% This would lead to a more reliable collection of studies in reviews and allow readers to compare multiple studies from multiple sources, rather than relying on one single study \cite{tranfield2003towards, hedges1992meta}.


% especially challenging given the increasing volume of information available to the average consumer \cite{tranfield2003towards}.
%information synthesis is becoming more difficult \cite{tranfield2003towards}. 
% Conflicting health information can also impair attention and increase confusion about the best course of action ~\cite{barnwell2022healthy}.


% Back to the general public, and their bias (can shorten)

%An essential aspect of scientific research is to communicate key findings to a broader audience for informed decision making.  
% Such effort has led to a remarkable improvement in societal decision-making.  
% For example, %in the medical domain, 
% according to reports by the CDC, 70\% of today's medical decisions are based on clinical laboratory test results \cite{cdc}, compared to the speculated 15-20\% in 1991 \cite{smith1991poverty}, which led to many ineffective patient treatments. 

% unlike scientists who synthesize prior evidence to contextualize their findings,


% \hari{How do experts/ scientists synthesize related/incremental evidence?} 





















% How do people make decisions? 

% It's not as simple as looking through a bunch of options.

% % For scientists
% for scientists, identifying a new research direction or making sense of existing findings and how they contribute to big-picture theories requires information synthesis.

% Again, because research is incremental, sometimes you will read about evidence supporting the thoery, sometimes you don't. 

% Scientists are trained to take into account of all sources of findings (some for, some against), to create new work. Value of review papers or reflective synthesis. 

% But we don't have a good idea of how exactly do scientists synthesize findings from existing work to identify research directions and revamp/update theories. It's a collective effort, but within one scientist, the process is not well modeled. 

% With more and more research out there, we need to start thinking about how we want to build tools to help scientists reconcile the increasing amount of knowledge. 

% Fields like information retrieval and HCI is working hard to figure out how can we make it easier for users to search for information and filter out misinformation,

% But without a formal model of how people synthesize information to make decisions, we don't know how to best help people better synthesize information.

% % For the general public
% This information synthesis problem is even more pressing for the general public.

% The average information consumer is not trained to think about the scientific methods. 

% So when scientists and journalists communicate incremental findings to the general public, people might not know how to digest/process/synthesis potentially conflicting information.
% As a results, they might make less-informed or biased choices.
% In scenarios related to public health and safety, this might have severe consequences. 

% Additionally, depending on the perspective of the source, the same dataset can be interpreted differently, And it's possible for your average information consumer to encounter conflicting argument (NYTUpshot example). 

% Goal 
% So ultimately, we as a field want to come up with visualization tools to help people better synthesize information and form mental representations that's less biased. 

% But we can't build such a tool without first understanding the underlying mechanisms of how people synthesize information. 

% For example, people have all sorts of biases when they process information (examples). -> people tend to heavily rely on their prior beliefs, confirmation bias, etc, So if we understand the mechanism, we can design tools to help them avoid these bias. 



 
 


% \hari{scratch notes for related work}
% \\
% Decision tree tool for selecting evidence synthesis method for environmental management decisions based on purpose of synthesis, required outcome and  decision constraints~\cite{cook2017simplifying}. \textbf{Purposes} of evidence synthesis:  assess causal associations, evaluate effectiveness, probability of success. \textbf{Desirable outcome}: confidence in conclusions/ how well conclusions can approximate the `truth.' \textit{Constraints:} time, technical expertise, Types of evidence synthesis: Narrative reviews, scoring, conceptual models, systematic maps, rapid reviews, stand-alone meta analysis, etc. 
% \\
% % Method for designing visualizations for decision-support based on Jen Rasmussen's abstraction-aggregation hierarchy.~\cite{rouse2017interactive}
% \\
% errors in theory-evidence coordination~\cite{shah2017makes}; Bias towards certainty--- interpret statements from reports as true vs. false. Avoiding conflicting information (need to process conflicting (with their beliefs) information at deeper level); Belief consistency; presence of visualizations triggers system 1 thinking--adds credibility. Numeracy and statistical reasoning skills.  
% \\
% Principles for systematic reviews~\cite{briner2012systematic}. Analysis and synthesis; analysis---examine and dissect individual studies and explore how the components relate to one another; synthesis---process of putting findings from individual studies together ``into a new or different arrangement and developing knowledge that is not apparent in reading individual studies in isolation'' Process: extracitng data from individual studies using data extraction forms. 
% \\
% 20 approaches to research synthesis~\cite{dixon2004integrative}
% \\
% Synthesis categories~\cite{rousseau200811}: aggregative, integrative, interpretation, and explanation. 
% \\
% presence of conflicting information impacts ability to judge veracity of news in systematic ways~\cite{karduni2018can}. 
% \\
% Integrating charts and captions- case study with line charts~\cite{kim2021towards}. When both charts and captions emphasize high-prominence features, readers take doubly emphasized high-prominence feature as takeaway; when the caption describes a low-prominence chart feature, readers rely on the chart and report a higher-prominence feature as the takeaway. We also find that external information that provides context, helps further convey the caption’s message to the reader.
% \\
% visual system can extract broad statistics from a display~\cite{franconeri2021science, szafir2016four}; -- statistics at a glance. 
% \\

% cognitive cost and benefits from using multiple-view vis: simultaneous more useful than sequential~\cite{jun2013exploring}. 



% % Yousif, S. R., Aboody, R., & Keil, F. C. (2019). The illusion of consensus: A failure to distinguish between true and false consensus. Psychological Science, 30(8), 1195-1204.

% Believability of consensus heuristics. Individuals are sensitive to consensus in a superficial rather than informative way. 


% % van Strien, J. L., Brand-Gruwel, S., & Boshuizen, H. P. (2014). Dealing with conflicting information from multiple nonlinear texts: Effects of prior attitudes. Computers in Human Behavior, 32, 101-111.


% students with strong attitudes took explicit stances and added large proportions of information not presented in the reading materials in their essays, whereas students with neutral attitudes wrote syntheses and borrowed more information from the materials.



% % Ciccione, L., & Dehaene, S. (2021). Can humans perform mental regression on a graph? Accuracy and bias in the perception of scatterplots. Cognitive Psychology, 128, 101406.

% Human adults could accurately judge if it was increasing or decreasing, fit a regression line, and extrapolate outside the original data range, for both linear and non-linear functions.  (regression. However, they overestimated the absolute value of the regression slope.)




% % Chen, M., & Jäenicke, H. (2010). An information-theoretic framework for visualization. IEEE Transactions on Visualization and Computer Graphics, 16(6), 1206-1215.

% Multi-view visualization is another means for error detection and correction, especially in visualizing non-spatial data, where errors are often due to the perceptual load of visual search, change detection
% and attention. 

% sensemaking

% % Patterson, R. E., Blaha, L. M., Grinstein, G. G., Liggett, K. K., Kaveney, D. E., Sheldon, K. C., ... & Moore, J. A. (2014). A human cognition framework for information visualization. Computers & Graphics, 42, 42-58.

% Leverage points: capture exogenous attention, endogenous attention, chunking, reasoning with mental models

% Sensemaking   (also Pirolli and Card)

% % Card, M. (1999). Readings in information visualization: using vision to think. Morgan Kaufmann.


% Sensemaking   (also Pirolli and Card)


% % Eberhard, K. (2021). The effects of visualization on judgment and decision-making: a systematic literature review. Management Review Quarterly, 1-48.



% that information visualization can improve decision quality as well as speed, with more mixed efects on other variables, for instance, decision confidence.


% % Isberner, M. B., Richter, T., Maier, J., Knuth-Herzig, K., Horz, H., & Schnotz, W. (2013). Comprehending conflicting science-related texts: graphs as plausibility cues. Instructional Science, 41(5), 849-872.

% Graphs can serve as plausibility cues and boost situation model strengths for texts which contain them. 

% % Rouse, W. B., Pennock, M. J., Oghbaie, M., & Liu, C. (2017). Interactive visualizations for decision support: Application of Rasmussen's abstraction-aggregation hierarchy. Applied ergonomics, 59, 541-553.

% % Liu, M.X. et al. (2019). Unakite: Scaffolding developers’ decision-making using the web. In Proceedings of the 32nd Annual ACM Symposium on User Interface Software and Technology (UIST '19). Association for Computing Machinery, New York, NY, USA, 67–80. DOI:https://doi.org/10.1145/3332165.3347908

% Unakite is a Chrome plug-in developed to help developers consider tradeoffs, synthesize information, and streamline decision-making when creating new software. Users can drag snippets of information found online to a comparison table that keeps track of findings and tradeoffs of specific features. A similar comparison table approach could help users synthesize heterogeneous evidence from multiple sources online. However, we first need to know more about how users perceive conflicting evidence from data visualizations to inform the design of such decision-making tools.

% % Tsetsos, K. Chater, N. & Usher, M. (2012). Salience driven value integration explains decision biases and preference reversal. Proceedings of the National Academy of Sciences, USA, 109, 9659–9664.

% Similar to order effects, high magnitude values are weighted more heavily when people must summarize multiple values presented over time. The salience of these events (first or peak event; high magnitude) explains their over-weighting.

% % Fisher, M. & Keil, F.C. (2018). The binary bias: A systematic distortion in the integration of information. Psychological Science, 29(11), 1846–1858.

% Participants synthesized 17 verbal claims about a given topic (e.g., whether or not a new medication causes hunger). The evidence varied in both direction (positive/neutral/negative) and strength (e.g., 2 times as likely, 4 times as likely). The distribution of these claims was purposely imbalanced across participants. People's posterior beliefs about a given claim were most strongly influenced by the imbalanced distribution of evidence claims. Additional studies using various data visualization formats (including histograms, pie charts and dot plots) showed that having an imbalanced distribution significantly influenced participants' estimates of the mean in graphs. These findings suggest that people use a binary bias when synthesizing multiple data points, which can distort their summaries of information. However, it is unclear if people are biased when summarizing visualized data even in cases where the distribution of heterogeneous evidence is balanced.

% % Koehler, D.J. & Pennycook, G. (2019). How the public, and scientists, perceive advancement of knowledge from conflicting study results. Judgment and Decision Making,  14(6),  671-682.

% Participants viewed two scientific findings that either agreed with or conflicted with one another. After seeing two conflicting findings, a large percentage of participants failed to endorse the view that 'we know more' as a result of the two findings. These findings suggest that non-scientists may not always perceive new findings as scientific progress and can actually interpret conflicting findings as a loss of scientific knowledge.











% \subsection{Visualizations in Science Reporting}




% Conflicting evidence 

% \subsection{Visual Information Synthesis and Sensemaking}

% Cognitive biases
% Mitigating biases via seeking/providing additional information 

% Learning Scienes/Writing - syntehzing text, refutation, creating argument 

% \subsection{Validating Evidence}

% Misinformation
% Comparisons



% While visualisations have been primarily used for 

% Visualisations are information dense. 

% Visualisations have percolated to day to day aspects of life. 

% Visualisation for information synthesis \cite{mcgill2022knowledge}

% Humans reading vis as a pipeline, and the complex visualization works together with human biases, creating noises that can interfere with information transmission to the end info consumer and harm understanding \cite{}

% \subsection{Visual and Text}

% \cite{powell2015clearer} - A clearer picture: The contribution of visuals and text to framing effects
% \cite{david1998news} - visualizations improve people's ability to recall content in news

% \subsection{Memory and Recall of Information}

% people tend to remember negative stimuli better than positive stimuli \cite{ohira1998effects}
% people remember text better when text is presented with visuals, compared to text alone \cite{tindall1997two}.
% titles influence the recall of main messages in visualizations \cite{kong2019trust}

% \subsection{Techniques to help people synthesize information}
% \cite{koytek2017mybrush} - brushing and linking vis techniques

% \subsection{Lit review - to be deleted later}
% %Key takeaways from lit review
% \begin{enumerate}
%     \item Reducing opinion polarization: Effects of exposure to similar people with differing political views \cite{balietti2021reducing} 
%     \begin{itemize}
%         \item Small but significant increase in support of redistribution across
%         \item Participants with mild views updated their stance asymmetrically in favor of redistributions
%         \item Folks with strong views became even more extreme when matched with same-stance other
%         \item Cross stance interactions depolarised strong views
%         \item Informal communication increases support for redistribution and reduces overall opinion polarisation
%         \item Increased closeness leads to larger stance updates
%         \item Exposure to political views influences feelings of closeness - Heider’s Balance theory and Festinger’s cognitive dissonance theory
%     \end{itemize}
%     \item Can you verifi this? studying uncertainty and decision-making about misinformation using visual analytics. \cite{karduni2018can}
%     \begin{itemize}
%         \item In general, cues have a significant effect on user’s fake prediction and accuracy
%         \item Opinionated, fear, social network - most important cues
%         \item Did not see confirmation bias - could be due to the user’s use of the app which made them slow down
%     \end{itemize}
%     \item The Illusion of Consensus: A failure to Distinguish Between True and False Consensus \cite{yousif2019illusion}
%     \begin{itemize}
%         \item Exp 1: No difference between true consensus and false consensus in confidence. (both false and true consensus higher than no consensus)
%         \item Exp 2: No difference between true consensus and false consensus in confidence,(both false and true consensus higher than no consensus) but confidence rating higher than experiment 1 \item Exp 3: No difference between true consensus and false consensus in confidence  (both false and true consensus higher than no consensus)
%         \item Exp 4: No difference between true consensus and false consensus in confidence -(both false and true consensus higher than no consensus) - cannot be explained by explicit beliefs.``Overall, 50\% of the participants believed that a true consensus was most believable, 16\% believed that a false consensus was most believable, and 33\% believed that both were equally believable”
%         \item Exp 5: Massive difference in true and false consensus. No difference between no and false consensus, except false had slightly higher confidence than no consensus

%     \end{itemize}
%     \item Dealing with conflicting information from multiple nonlinear texts: Effects of prior attitudes \cite{van2014dealing}
%     \begin{itemize}
%         \item Boys were significantly more favorable of violent video games
%         \item Prior attitude (? or is it prior knowledge?) was significantly associated with the proportion of added content (and not opinion statements)
%         \item Students with prior attitudes defended a stance, but those with neutral attitudes made summaries or synthesis i.e. Prior attitudes promotes certain approaches to writing tasks - Students with neutral attitudes were more likely to say that the information presented was inconclusive


%     \end{itemize}
%     \item Topic-based Exploration and Embedded Visualizations for Research Idea Generation \cite{guo2018topic}
%     \begin{itemize}
%         \item Identified 4 categories of sensemaking activities
%         \begin{itemize}
%             \item Seeking a new frame / reframing
%             \item Questioning / preserving the frame
%             \item Seeking and filtering data
%             \item Discovering new data or relationships
%         \end{itemize}
%         \item Identified challenges and frustrations experienced by researchers
%         \begin{itemize}
%             \item Context switch: Switching back and forth between literature search and the writing process or multiple threads of related work costs additional mental energy
%             \item Evidence imbalance: Evidence inconsistent with a proposal`s hypotheses and arguments is less likely to be discovered and considered during the proposal writing process
%             \item Disciplinary barriers: Users are less likely to discover publications relevant to a proposal but from a less familiar research area
%             \item Citation based clusters: Citation relationships, while used extensively by the participants, do not guarantee relevance or comprehensive coverage of related work

%         \end{itemize}
%     \end{itemize}
 
% \end{enumerate}


% We will discuss the experimental stimuli in more details in Section \ref{StudyOverview}, and point to potential limitations and future directions in Section \ref{limitationsFuture}. 

% To account for these biases, in our present experiment, we carefully control for the order of the stimuli, kept chart type constant, adding lines and dots in the chart to provide mulitple chanels of a, covered different 'categories' of slopes,
% didn't include a title in the intiial phases, but included a title later one to test for geenralizability 
% no addigional pictures, no colors,

% Effect of title
%  One study found that visualizations with a title showed higher quality memory reports for their content, especially when the title included ‘message redundancy,’ an additional section of text that focused the viewer on a key pattern in the visualization \cite{borkin2015beyond}.
 % slanted titles \cite{kong2018frames}

% Context matters
% additional images matter - Bateman et al. found that visualizations that integrate data with illustrations yielded better memory of the data compared to minimalistic outlines of bar charts  \cite{bateman2010useful}
% another study showed that graphs with ‘data redundancy’ – symbolic numbers placed on or near visual marks that already show those numbers visually – actually showed \textit{higher} quality memory reports for their content \cite{borkin2015beyond}.
% Borkin et al. found a related result – that people can better recall having seen a visualization that includes pictures [4], though it is not clear if they would better recall the data, per se.
% When images and clip-art are embedded in the visualization’s data representation, Borgo et al. found occasional impact to work- \cite{borgo2012empirical}
% When memory is crowded, similar information, such as verbal code for one set of numbers and verbal code for a second set of numbers, interferes adn becomes noisy or lost -> Time, number and length: Similarities and differences in discrimination in adults and children
% \cite{droit2008time}




% In a real world scenario, synthesising information happens with information coming from different sources, and in different modalities (e.g., textual, data visualizations, videos, audios etc.). As per persuasion literature - the source, message, and receiver characteristics will play an important role in how this information affects the receiver \cite{ajzen1992persuasive, o2015persuasion}.(Communication literature refers to information consumers as information receivers, but we will refer to them as consumers throughout the document for consistency).

% Consumer characteristics like prior knowledge, beliefs, motivation\cite{pandey2014persuasive, xiong2019curse}, different abilities or skills like reasoning \cite{schweinsberg2021same}, visual literacy\cite{franconeri2021science}, knowledge of statistics \cite{hofman2020visualizing}, and the social context\cite{barnlund2017transactional} the message is situated in, among many others affect the persuasive power of the message. 

% Pandey et al. 2014 \cite{pandey2014persuasive} argues that a message needs to have at least three characteristics - 1. Contextual information; 2. Evidence or the argument 3. Data provided in support of the evidence. For Experiment 1, we only provided the data devoid of any contextual information to the participants, which sets the baseline for how visual information synthesis can take place. %if the visual information is provided without any context or argument.
% In Experiment 2, we provided our participants with contextual information via two real world scenarios, but without any argument or interpretation of what the data is saying. 
% % For this Experiment, we provided our participants with two real world scenarios devoid of any argument. 

% For Experiment 3, we provided all three necessary information points - the context, the argument, and data to support the argument to create a real world scenario. This was achieved by providing the participants with two news articles providing with an interpretation what the data means. As involvement with the message has been argued to have an effect on the motivation\cite{pandey2014persuasive, luo2019motivated}, we chose a scenario of potential relevance to the participants - relationship between quality of life and public spending. Moreover, visualizations are often studied independently of their context, even though in real-world scenarios they appear with text. In many visualization studies about data storytelling, e.g., \cite{ajani2021declutter, borkin2013makes}, visualizations are used as a stimuli separated from the text of the story. Experiment 3 help us understand the impact of visualization integrated with text, which simulates real world scenarios better, and increases the ecological validity of the work. Our Experimental stimuli, analysis, and data can be found at \url{https://osf.io/pc3f7/}(Here on referred to as supplementary material)

% \cx{visualizations are often studied independently of their context, even though in real-world scenarios they appear with text. In many visualization studies about data storytelling, e.g., \cite{ajani2021declutter, borkin2013makes}, visualizations are used as a stimuli separated from the text of the story. Exp 3 help us understand the impact of visualization integrated with text, which simulates real world scenarios better, and increases the ecological validity of the work. }

% \cx{might want to say why we wrote the articles ourselves - to ensure people never read it before, more precise control over characteristics of the articles, such as variations and similarities between different Conditions, } \prateek{Does the following paragraph work?}



% \cx{Say our Experimental stimuli and analysis and data can be found at \url{...} and link your supplementary OSF page here!!!}



\subsection{Information Synthesis and Decision Making}


% \hari{scratch notes for related work}
% \\
% Decision tree tool for selecting evidence synthesis method for environmental management decisions based on purpose of synthesis, required outcome and  decision constraints~\cite{cook2017simplifying}. \textbf{Purposes} of evidence synthesis:  assess causal associations, evaluate effectiveness, probability of success. \textbf{Desirable outcome}: confidence in conclusions/ how well conclusions can approximate the `truth.' \textit{Constraints:} time, technical expertise, Types of evidence synthesis: Narrative reviews, scoring, conceptual models, systematic maps, rapid reviews, stand-alone meta analysis, etc. 
% \\
% % Method for designing visualizations for decision-support based on Jen Rasmussen's abstraction-aggregation hierarchy.~\cite{rouse2017interactive}
% \\
% errors in theory-evidence coordination~\cite{shah2017makes}; Bias towards certainty--- interpret statements from reports as true vs. false. Avoiding conflicting information (need to process conflicting (with their beliefs) information at deeper level); Belief consistency; presence of visualizations triggers system 1 thinking--adds credibility. Numeracy and statistical reasoning skills.  
% \\
% Principles for systematic reviews~\cite{briner2012systematic}. Analysis and synthesis; analysis---examine and dissect individual studies and explore how the components relate to one another; synthesis---process of putting findings from individual studies together ``into a new or different arrangement and developing knowledge that is not apparent in reading individual studies in isolation'' Process: extracitng data from individual studies using data extraction forms. 
% \\
% 20 approaches to research synthesis~\cite{dixon2004integrative}
% \\
% Synthesis categories~\cite{rousseau200811}: aggregative, integrative, interpretation, and explanation. 
% \\
% presence of conflicting information impacts ability to judge veracity of news in systematic ways~\cite{karduni2018can}. 
% \\
% Integrating charts and captions- case study with line charts~\cite{kim2021towards}. When both charts and captions emphasize high-prominence features, readers take doubly emphasized high-prominence feature as takeaway; when the caption describes a low-prominence chart feature, readers rely on the chart and report a higher-prominence feature as the takeaway. We also find that external information that provides context, helps further convey the caption’s message to the reader.
% \\
% visual system can extract broad statistics from a display~\cite{franconeri2021science, szafir2016four}; -- statistics at a glance. 
% \\

% cognitive cost and benefits from using multiple-view vis: simultaneous more useful than sequential~\cite{jun2013exploring}. 

\subsection{Processing Conflicting Information}
Prior research has investigated conflicting information as a \textit{selection} problem and highlighted numerous biases in how people choose between information sources. A widely prevalent behavior is \textit{confirmation bias} in which readers favor confirmation-seeking information over contradicting information~\cite{klayman1995varieties, charness2021people, knobloch2020confirmation, knobloch2012preelection}. 







% Charness, G., Oprea, R., & Yuksel, S. (2021). How do people choose between biased information sources? Evidence from a laboratory experiment. Journal of the European Economic Association, 19(3), 1656-1691.

Often times people have prior knowledge and beliefs. When presented with information with opposing bias, participants favor confirmation-seeking information (the reason is selecting information that is more accurate ex-ante, conflates guessing accuracy with signal accuracy) rather than contradicting information (seeking signals that go against priors). 

% Hart, W., Albarracín, D., Eagly, A. H., Brechan, I., Lindberg, M. J., & Merrill, L. (2009). Feeling validated versus being correct: a meta-analysis of selective exposure to information. Psychological bulletin, 135(4), 555.

Congeniality bias moderated by variables that affect the strength of participants’s defense motivation and accuracy of motivation. 


% Garz, M., Sood, G., Stone, D. F., & Wallace, J. (2020). The supply of media slant across outlets and demand for slant within outlets: Evidence from US presidential campaign news. European Journal of Political Economy, 63, 101877.

For news outlets with partisan reputations, the news is slanted congenially for typical readers. Within-outlets, stories more congenial to a typical reader are not more popular.  Democrats are willing to get news from NYT when it was uncongenial, but R unwilling to NYT even when congenial. But R willing to click on uncongenial Fox stories. — strong within outlet demand for news regardless of its congeniality. 

Measure clicks

% Kong, H. K., Liu, Z., & Karahalios, K. (2018, April). Frames and slants in titles of visualizations on controversial topics. In Proceedings of the 2018 CHI conference on human factors in computing systems (pp. 1-12).

Slant of the visualization title influenced the perceived main message of a visualization, with viewers deriving opposing messages from the same visualizations. 

% Lauer, C., & O'Brien, S. (2020). How people are influenced by deceptive tactics in everyday charts and graphs. IEEE Transactions on Professional Communication, 63(4), 327-340.

Deceptive tactics (inverted axis– message reversal, message exaggeration–truncated y-axis, title slants ) caused participants to misinterpret information across all graph types. 

% Richter, T., & Maier, J. (2017). Comprehension of multiple documents with conflicting information: A two-step model of validation. Educational psychologist, 52(3), 148-166.

Readers' prior beliefs may lead to biased processing of conflicting information and a one-sided mental model of controversial issues (text-belief consistency effects).  Two-step model of processing conflicting information. Detection of belief-inconsistent information  → strategic elaboration of inconsistencies

% Poeple do this in text, how about vis?
% Ford, N. (2004). Modeling cognitive processes in information seeking: From Popper to Pask. Journal of the American Society for Information Science and Technology, 55(9), 769-782.

Uncertainty as a driver of information seeking. The uncertainty is potentially resolved as a result of acquisition and processing new information. 

% Karduni, A., Markant, D., Wesslen, R., & Dou, W. (2020). A Bayesian cognition approach for belief updating of correlation judgement through uncertainty visualizations. IEEE Transactions on Visualization and Computer Graphics, 27(2), 978-988.

Visualization with uncertainty led to less belief updating compared to visualizations without uncertainty, especially when presented with correlation visualization that is incongruent with prior beliefs. 


% Yousif, S. R., Aboody, R., & Keil, F. C. (2019). The illusion of consensus: A failure to distinguish between true and false consensus. Psychological Science, 30(8), 1195-1204.

Believability of consensus heuristics. Individuals are sensitive to consensus in a superficial rather than informative way. 


% van Strien, J. L., Brand-Gruwel, S., & Boshuizen, H. P. (2014). Dealing with conflicting information from multiple nonlinear texts: Effects of prior attitudes. Computers in Human Behavior, 32, 101-111.


students with strong attitudes took explicit stances and added large proportions of information not presented in the reading materials in their essays, whereas students with neutral attitudes wrote syntheses and borrowed more information from the materials.

% Fisher, M., & Keil, F. C. (2018). The binary bias: A systematic distortion in the integration of information. Psychological Science, 29(11), 1846-1858.

When summarizing evidence, people exhibit a binary bias: a tendency to impose categorical distinctions on continuous data. The binary bias distorts belief formation—such that when people aggregate conflicting scientific reports, they attend to valence and inaccurately weight the extremity of the evidence.
The same effect occurs when people interpret popular forms of data visualization, and it cannot be explained by other statistical features of the stimuli.

the binary bias again explained estimates of the mean above and beyond the influence of other statistical features.

% Ciccione, L., & Dehaene, S. (2021). Can humans perform mental regression on a graph? Accuracy and bias in the perception of scatterplots. Cognitive Psychology, 128, 101406.

Human adults could accurately judge if it was increasing or decreasing, fit a regression line, and extrapolate outside the original data range, for both linear and non-linear functions.  (regression. However, they overestimated the absolute value of the regression slope.)

% Ericson, J. D., Albert, W. S., & Duane, J. N. (2022). Political affiliation moderates subjective interpretations of COVID-19 graphs. Big data & society, 9(1), 20539517221080678.

(a) COVID-19 data or (b) COVID-19 data labeled ‘Influenza (Flu)’. Block 1 examined responses to cross-sectional mortality data (bar graphs, treemaps); results revealed that perceptual estimates comparing mortality in two countries were similar across political affiliations and chart types (all ps>.05), while subjective judgments revealed a disease x political party interaction (p<.05). Although Democrats and Republicans provided similar proportion estimates, Democrats interpreted mortality to be higher than Republicans; Democrats also interpreted mortality to be higher for COVID-19 than Influenza. . Democrats and Republicans indicated similar subjective rates of change for COVID-19 trends, and Democrats indicated lower subjective rates of change for Influenza than in any other condition. Thus, while Democrats and Republicans saw the graphs similarly in terms of percentages and line slopes, their subjective interpretations diverged.


% Chen, M., & Jäenicke, H. (2010). An information-theoretic framework for visualization. IEEE Transactions on Visualization and Computer Graphics, 16(6), 1206-1215.

Multi-view visualization is another means for error detection and correction, especially in visualizing non-spatial data, where errors are often due to the perceptual load of visual search, change detection
and attention. 

sensemaking

% Patterson, R. E., Blaha, L. M., Grinstein, G. G., Liggett, K. K., Kaveney, D. E., Sheldon, K. C., ... & Moore, J. A. (2014). A human cognition framework for information visualization. Computers & Graphics, 42, 42-58.

Leverage points: capture exogenous attention, endogenous attention, chunking, reasoning with mental models

Sensemaking   (also Pirolli and Card)

% Card, M. (1999). Readings in information visualization: using vision to think. Morgan Kaufmann.


Sensemaking   (also Pirolli and Card)


% Eberhard, K. (2021). The effects of visualization on judgment and decision-making: a systematic literature review. Management Review Quarterly, 1-48.



that information visualization can improve decision quality as well as speed, with more mixed efects on other variables, for instance, decision confidence.


% Isberner, M. B., Richter, T., Maier, J., Knuth-Herzig, K., Horz, H., & Schnotz, W. (2013). Comprehending conflicting science-related texts: graphs as plausibility cues. Instructional Science, 41(5), 849-872.

Graphs can serve as plausibility cues and boost situation model strengths for texts which contain them. 

% Rouse, W. B., Pennock, M. J., Oghbaie, M., & Liu, C. (2017). Interactive visualizations for decision support: Application of Rasmussen's abstraction-aggregation hierarchy. Applied ergonomics, 59, 541-553.














\subsection{Visualizations in Science Reporting}




Conflicting evidence 

\subsection{Visual Information Synthesis and Sensemaking}

Cognitive biases
Mitigating biases via seeking/providing additional information 

Learning Scienes/Writing - syntehzing text, refutation, creating argument 

\subsection{Validating Evidence}

Misinformation
Comparisons



While visualisations have been primarily used for 

Visualisations are information dense. 

Visualisations have percolated to day to day aspects of life. 

Visualisation for information synthesis \cite{mcgill2022knowledge}

Humans reading vis as a pipeline, and the complex visualization works together with human biases, creating noises that can interfere with information transmission to the end info consumer and harm understanding \cite{}

\subsection{Visual and Text}

\cite{powell2015clearer} - A clearer picture: The contribution of visuals and text to framing effects
\cite{david1998news} - visualizations improve people's ability to recall content in news

\subsection{Memory and Recall of Information}

people tend to remember negative stimuli better than positive stimuli \cite{ohira1998effects}
people remember text better when text is presented with visuals, compared to text alone \cite{tindall1997two}.
titles influence the recall of main messages in visualizations \cite{kong2019trust}

\subsection{Techniques to help people synthesize information}
\cite{koytek2017mybrush} - brushing and linking vis techniques

\subsection{Lit review - to be deleted later}
%Key takeaways from lit review
\begin{enumerate}
    \item Reducing opinion polarization: Effects of exposure to similar people with differing political views \cite{balietti2021reducing} 
    \begin{itemize}
        \item Small but significant increase in support of redistribution across
        \item Participants with mild views updated their stance asymmetrically in favor of redistributions
        \item Folks with strong views became even more extreme when matched with same-stance other
        \item Cross stance interactions depolarised strong views
        \item Informal communication increases support for redistribution and reduces overall opinion polarisation
        \item Increased closeness leads to larger stance updates
        \item Exposure to political views influences feelings of closeness - Heider’s Balance theory and Festinger’s cognitive dissonance theory
    \end{itemize}
    \item Can you verifi this? studying uncertainty and decision-making about misinformation using visual analytics. \cite{karduni2018can}
    \begin{itemize}
        \item In general, cues have a significant effect on user’s fake prediction and accuracy
        \item Opinionated, fear, social network - most important cues
        \item Did not see confirmation bias - could be due to the user’s use of the app which made them slow down
    \end{itemize}
    \item The Illusion of Consensus: A failure to Distinguish Between True and False Consensus \cite{yousif2019illusion}
    \begin{itemize}
        \item Exp 1: No difference between true consensus and false consensus in confidence. (both false and true consensus higher than no consensus)
        \item Exp 2: No difference between true consensus and false consensus in confidence,(both false and true consensus higher than no consensus) but confidence rating higher than experiment 1 \item Exp 3: No difference between true consensus and false consensus in confidence  (both false and true consensus higher than no consensus)
        \item Exp 4: No difference between true consensus and false consensus in confidence -(both false and true consensus higher than no consensus) - cannot be explained by explicit beliefs.``Overall, 50\% of the participants believed that a true consensus was most believable, 16\% believed that a false consensus was most believable, and 33\% believed that both were equally believable”
        \item Exp 5: Massive difference in true and false consensus. No difference between no and false consensus, except false had slightly higher confidence than no consensus

    \end{itemize}
    \item Dealing with conflicting information from multiple nonlinear texts: Effects of prior attitudes \cite{van2014dealing}
    \begin{itemize}
        \item Boys were significantly more favorable of violent video games
        \item Prior attitude (? or is it prior knowledge?) was significantly associated with the proportion of added content (and not opinion statements)
        \item Students with prior attitudes defended a stance, but those with neutral attitudes made summaries or synthesis i.e. Prior attitudes promotes certain approaches to writing tasks - Students with neutral attitudes were more likely to say that the information presented was inconclusive


    \end{itemize}
    \item Topic-based Exploration and Embedded Visualizations for Research Idea Generation \cite{guo2018topic}
    \begin{itemize}
        \item Identified 4 categories of sensemaking activities
        \begin{itemize}
            \item Seeking a new frame / reframing
            \item Questioning / preserving the frame
            \item Seeking and filtering data
            \item Discovering new data or relationships
        \end{itemize}
        \item Identified challenges and frustrations experienced by researchers
        \begin{itemize}
            \item Context switch: Switching back and forth between literature search and the writing process or multiple threads of related work costs additional mental energy
            \item Evidence imbalance: Evidence inconsistent with a proposal`s hypotheses and arguments is less likely to be discovered and considered during the proposal writing process
            \item Disciplinary barriers: Users are less likely to discover publications relevant to a proposal but from a less familiar research area
            \item Citation based clusters: Citation relationships, while used extensively by the participants, do not guarantee relevance or comprehensive coverage of related work

        \end{itemize}
    \end{itemize}
 
\end{enumerate}






\subsection{Visual Perception, Memory, and Recall}



